Evaluating the Rationale Understanding of Critical Reasoning in Logical Reading Comprehension

To precisely evaluate a language model's capability for logical reading comprehension, we present a dataset for testing the understanding of the rationale behind critical reasoning. For questions taken from an existing multiplechoice logical reading comprehension dataset, we crowdsource rationale texts that explain why we should select or eliminate answer options, resulting in 3,003 multiple-choice subquestions that are associated with 943 main questions. Experiments on our dataset show that recent large language models (e.g., InstructGPT) struggle to answer the subquestions even if they are able to answer the main questions correctly. We find that the models perform particularly poorly in answering subquestions written for the incorrect options of the main questions, implying that the models have a limited capability for explaining why incorrect alternatives should be eliminated. These results suggest that our dataset encourages further investigation into the critical reasoning ability of language models while focusing on the elimination process of relevant alternatives.

==> tables/main_result_full.tex <==
\begin{tabular}{lcrrrrrr} \toprule
\textbf{Model} & \textbf{\# Param} & \makecell[c]{\textbf{MainQ}\\\textbf{Accuracy}} & \makecell[c]{\textbf{SubQ}\\\textbf{Accuracy}} & \makecell[c]{\textbf{Correct Opt.}\\\textbf{Accuracy}} & \makecell[c]{\textbf{Incorrect Opt.}\\\textbf{Accuracy}} & \textbf{Consist.} &  \makecell[r]{\textbf{MainQ-wise}\\\textbf{Accuracy}} \\ \midrule
\multicolumn{8}{c}{\cellcolor{light-gray} \emph{Fully Supervised on ReClor}} \\
%\textsc{DeBERTa-v3-Large} & 304M & 66.0\hphantom{$_{\pm0.00}$} & 33.1\hphantom{$_{\pm0.00}$} & 56.1\hphantom{$_{\pm0.00}$} & 25.0\hphantom{$_{\pm0.00}$} & 2.4 & 32.8\\
%\textsc{UnifiedQA-v2-Base} & 220M & 40.5\hphantom{$_{\pm0.00}$} & 25.8\hphantom{$_{\pm0.00}$} & 21.3\hphantom{$_{\pm0.00}$} & 27.4\hphantom{$_{\pm0.00}$} & 0.7 & 26.0\\
%\textsc{UnifiedQA-v2-Large} & 770M & 57.7\hphantom{$_{\pm0.00}$} & 25.0\hphantom{$_{\pm0.00}$} & 19.9\hphantom{$_{\pm0.00}$} & 26.8\hphantom{$_{\pm0.00}$} & 1.4 & 24.7\\
%\textsc{UnifiedQA-v2-3B} & 3B & 66.8\hphantom{$_{\pm0.00}$} & 25.3\hphantom{$_{\pm0.00}$} & 21.8\hphantom{$_{\pm0.00}$} & 26.6\hphantom{$_{\pm0.00}$} & 1.4 & 25.2\\
\multicolumn{8}{c}{\cellcolor{light-gray} \emph{Five-Shot on ReClor}} \\
\textsc{Flan-UL2} & 20B & 58.5$_{\pm0.3\hphantom{0}}$ & 65.5$_{\pm5.1\hphantom{0}}$ & 88.0$_{\pm4.0\hphantom{0}}$ & 57.6$_{\pm5.4\hphantom{0}}$ & 16.9 & 64.3\\
\textsc{LLaMA 7B} & 7B & 25.8$_{\pm1.6\hphantom{0}}$ & 28.6$_{\pm7.1\hphantom{0}}$ & 39.8$_{\pm13.1}$ & 24.6$_{\pm6.3\hphantom{0}}$ & 0.8 & 28.2\\
\textsc{LLaMA 13B} & 13B & 38.7$_{\pm2.7\hphantom{0}}$ & 36.3$_{\pm3.5\hphantom{0}}$ & 63.6$_{\pm4.0\hphantom{0}}$ & 26.6$_{\pm3.6\hphantom{0}}$ & 2.9 & 36.6\\
\textsc{LLaMA 33B} & 33B & 58.5$_{\pm1.2\hphantom{0}}$ & 48.1$_{\pm3.5\hphantom{0}}$ & 77.3$_{\pm3.6\hphantom{0}}$ & 37.7$_{\pm3.6\hphantom{0}}$ & 6.2 & 48.0\\
\textsc{LLaMA 65B} & 65B & 69.1$_{\pm0.9\hphantom{0}}$ & 55.3$_{\pm2.7\hphantom{0}}$ & 85.0$_{\pm1.4\hphantom{0}}$ & 44.8$_{\pm2.5\hphantom{0}}$ & 11.2 & 54.9\\
\textsc{Vicuna 7B} & 7B & 33.4$_{\pm2.6\hphantom{0}}$ & 38.6$_{\pm3.3\hphantom{0}}$ & 61.4$_{\pm5.8\hphantom{0}}$ & 30.5$_{\pm3.4\hphantom{0}}$ & 2.8 & 38.3\\
\textsc{Vicuna 13B} & 13B & 46.2$_{\pm0.7\hphantom{0}}$ & 50.0$_{\pm4.4\hphantom{0}}$ & 78.2$_{\pm3.0\hphantom{0}}$ & 40.1$_{\pm4.6\hphantom{0}}$ & 5.6 & 49.4\\
\textsc{InstructGPT} & N/A & 71.8$_{\pm1.0\hphantom{0}}$ & 65.3$_{\pm1.8\hphantom{0}}$ & 88.4$_{\pm2.5\hphantom{0}}$ & 57.1$_{\pm1.5\hphantom{0}}$ & 18.2 & 64.0\\
\textsc{InstructGPT + CoT} & N/A & 67.8$_{\pm0.5\hphantom{0}}$ & 63.2$_{\pm2.1\hphantom{0}}$ & 88.5$_{\pm2.5\hphantom{0}}$ & 54.2$_{\pm2.8\hphantom{0}}$ & 17.2 & 61.8\\
\textsc{LLaMA2 7B} & 7B & 36.4$_{\pm2.1\hphantom{0}}$ & 35.2$_{\pm3.9\hphantom{0}}$ & 63.6$_{\pm6.5\hphantom{0}}$ & 25.1$_{\pm3.2\hphantom{0}}$ & 1.7 & 35.6\\
\textsc{LLaMA2 13B} & 13B & 48.5$_{\pm2.5\hphantom{0}}$ & 44.6$_{\pm3.2\hphantom{0}}$ & 75.3$_{\pm3.4\hphantom{0}}$ & 33.8$_{\pm4.0\hphantom{0}}$ & 5.3 & 44.7\\
\textsc{LLaMA2 70B} & 70B & 80.3$_{\pm0.4\hphantom{0}}$ & 60.0$_{\pm2.6\hphantom{0}}$ & 90.0$_{\pm1.1\hphantom{0}}$ & 49.4$_{\pm2.9\hphantom{0}}$ & 17.7 & 59.3\\
\textsc{Mistral 7B} & 7B & 59.9$_{\pm0.9\hphantom{0}}$ & 55.3$_{\pm3.4\hphantom{0}}$ & 83.6$_{\pm3.4\hphantom{0}}$ & 45.4$_{\pm3.6\hphantom{0}}$ & 9.0 & 54.4\\
\multicolumn{8}{c}{\cellcolor{light-gray} \emph{One-Shot on ReClor}} \\
%\textsc{UnifiedQA-v2-Base} & 220M & 27.4$_{\pm1.4\hphantom{0}}$ & 34.7$_{\pm6.4\hphantom{0}}$ & 42.8$_{\pm7.7\hphantom{0}}$ & 31.9$_{\pm6.2\hphantom{0}}$ & 0.7 & 34.6\\
%\textsc{UnifiedQA-v2-Large} & 770M & 27.1$_{\pm1.7\hphantom{0}}$ & 28.0$_{\pm4.7\hphantom{0}}$ & 29.2$_{\pm5.3\hphantom{0}}$ & 27.6$_{\pm4.9\hphantom{0}}$ & 0.0 & 27.6\\
%\textsc{UnifiedQA-v2-3B} & 3B & 31.3$_{\pm3.2\hphantom{0}}$ & 26.2$_{\pm2.8\hphantom{0}}$ & 26.0$_{\pm9.8\hphantom{0}}$ & 26.2$_{\pm1.4\hphantom{0}}$ & 0.3 & 26.1\\
%\textsc{UnifiedQA-v2-11B} & 11B & 44.1$_{\pm5.9\hphantom{0}}$ & 37.2$_{\pm7.4\hphantom{0}}$ & 53.8$_{\pm16.6}$ & 31.4$_{\pm4.4\hphantom{0}}$ & 2.0 & 36.5\\
\textsc{Flan-T5-XXL} & 11B & 61.3$_{\pm0.3\hphantom{0}}$ & 63.7$_{\pm3.7\hphantom{0}}$ & 85.9$_{\pm2.6\hphantom{0}}$ & 55.9$_{\pm3.9\hphantom{0}}$ & 14.0 & 62.5\\
\textsc{Flan-UL2} & 20B & 58.0$_{\pm0.5\hphantom{0}}$ & 66.0$_{\pm5.3\hphantom{0}}$ & 87.4$_{\pm3.9\hphantom{0}}$ & 58.5$_{\pm5.7\hphantom{0}}$ & 17.7 & 65.1\\
\textsc{LLaMA 7B} & 7B & 26.6$_{\pm0.9\hphantom{0}}$ & 32.4$_{\pm4.2\hphantom{0}}$ & 50.7$_{\pm11.1}$ & 26.1$_{\pm3.7\hphantom{0}}$ & 1.6 & 32.5\\
\textsc{LLaMA 13B} & 13B & 32.7$_{\pm2.4\hphantom{0}}$ & 33.8$_{\pm1.9\hphantom{0}}$ & 56.0$_{\pm5.8\hphantom{0}}$ & 26.0$_{\pm2.5\hphantom{0}}$ & 1.4 & 34.1\\
\textsc{LLaMA 33B} & 33B & 56.1$_{\pm1.0\hphantom{0}}$ & 49.3$_{\pm4.3\hphantom{0}}$ & 80.1$_{\pm3.8\hphantom{0}}$ & 38.5$_{\pm4.3\hphantom{0}}$ & 7.4 & 49.6\\
\textsc{LLaMA 65B} & 65B & 65.2$_{\pm1.4\hphantom{0}}$ & 52.6$_{\pm3.4\hphantom{0}}$ & 85.2$_{\pm1.3\hphantom{0}}$ & 41.1$_{\pm4.3\hphantom{0}}$ & 9.4 & 51.9\\
\textsc{Vicuna 7B} & 7B & 35.8$_{\pm2.0\hphantom{0}}$ & 38.9$_{\pm2.2\hphantom{0}}$ & 65.3$_{\pm3.1\hphantom{0}}$ & 29.5$_{\pm2.3\hphantom{0}}$ & 1.8 & 38.1\\
\textsc{Vicuna 13B} & 13B & 42.5$_{\pm0.8\hphantom{0}}$ & 45.2$_{\pm3.1\hphantom{0}}$ & 72.1$_{\pm3.3\hphantom{0}}$ & 35.8$_{\pm4.0\hphantom{0}}$ & 4.2 & 45.1\\
\textsc{InstructGPT} & N/A & 67.8$_{\pm0.5\hphantom{0}}$ & 64.6$_{\pm1.9\hphantom{0}}$ & 87.8$_{\pm2.0\hphantom{0}}$ & 56.3$_{\pm1.8\hphantom{0}}$ & 17.5 & 63.6\\
\textsc{InstructGPT + CoT} & N/A & 64.3$_{\pm2.5\hphantom{0}}$ & 64.3$_{\pm2.4\hphantom{0}}$ & 88.8$_{\pm1.3\hphantom{0}}$ & 55.7$_{\pm2.5\hphantom{0}}$ & 15.4 & 62.5\\
\textsc{LLaMA2 7B} & 7B & 35.0$_{\pm1.1\hphantom{0}}$ & 34.8$_{\pm2.4\hphantom{0}}$ & 61.7$_{\pm4.2\hphantom{0}}$ & 25.2$_{\pm2.6\hphantom{0}}$ & 2.2 & 35.2\\
\textsc{LLaMA2 13B} & 13B & 46.4$_{\pm2.4\hphantom{0}}$ & 43.7$_{\pm2.9\hphantom{0}}$ & 72.6$_{\pm3.6\hphantom{0}}$ & 33.4$_{\pm2.8\hphantom{0}}$ & 4.7 & 43.6\\
\textsc{LLaMA2 70B} & 70B & 77.2$_{\pm0.2\hphantom{0}}$ & 61.3$_{\pm0.7\hphantom{0}}$ & 90.0$_{\pm1.4\hphantom{0}}$ & 51.2$_{\pm1.2\hphantom{0}}$ & 20.0 & 61.0\\
\textsc{Mistral 7B} & 7B & 52.6$_{\pm1.4\hphantom{0}}$ & 53.4$_{\pm2.3\hphantom{0}}$ & 81.9$_{\pm2.8\hphantom{0}}$ & 43.4$_{\pm2.7\hphantom{0}}$ & 7.4 & 52.7\\
\multicolumn{8}{c}{\cellcolor{light-gray} \emph{Five-Shot on RULE}} \\
\textsc{Flan-UL2} & 20B & 57.9$_{\pm0.2\hphantom{0}}$ & 66.0$_{\pm4.9\hphantom{0}}$ & 87.7$_{\pm4.6\hphantom{0}}$ & 58.4$_{\pm5.0\hphantom{0}}$ & 17.8 & 64.9\\
\textsc{LLaMA 7B} & 7B & 29.1$_{\pm2.3\hphantom{0}}$ & 34.9$_{\pm2.5\hphantom{0}}$ & 64.3$_{\pm4.3\hphantom{0}}$ & 24.5$_{\pm2.4\hphantom{0}}$ & 1.5 & 35.5\\
\textsc{LLaMA 13B} & 13B & 36.8$_{\pm3.5\hphantom{0}}$ & 35.6$_{\pm2.5\hphantom{0}}$ & 68.1$_{\pm3.0\hphantom{0}}$ & 24.2$_{\pm2.8\hphantom{0}}$ & 2.4 & 36.0\\
\textsc{LLaMA 33B} & 33B & 53.6$_{\pm0.4\hphantom{0}}$ & 47.8$_{\pm4.5\hphantom{0}}$ & 77.8$_{\pm3.9\hphantom{0}}$ & 37.2$_{\pm4.8\hphantom{0}}$ & 5.7 & 47.6\\
\textsc{LLaMA 65B} & 65B & 66.2$_{\pm0.7\hphantom{0}}$ & 58.9$_{\pm6.3\hphantom{0}}$ & 86.5$_{\pm1.7\hphantom{0}}$ & 49.1$_{\pm7.6\hphantom{0}}$ & 12.0 & 58.0\\
\textsc{Vicuna 7B} & 7B & 35.0$_{\pm1.1\hphantom{0}}$ & 39.9$_{\pm3.9\hphantom{0}}$ & 60.2$_{\pm8.9\hphantom{0}}$ & 32.7$_{\pm4.4\hphantom{0}}$ & 3.2 & 39.8\\
\textsc{Vicuna 13B} & 13B & 43.9$_{\pm1.3\hphantom{0}}$ & 44.2$_{\pm2.7\hphantom{0}}$ & 72.6$_{\pm2.6\hphantom{0}}$ & 34.2$_{\pm2.6\hphantom{0}}$ & 4.1 & 44.0\\
\textsc{InstructGPT} & N/A & 70.2$_{\pm0.4\hphantom{0}}$ & 70.1$_{\pm2.3\hphantom{0}}$ & 90.0$_{\pm3.5\hphantom{0}}$ & 63.0$_{\pm2.0\hphantom{0}}$ & 23.1 & 69.2\\
\textsc{InstructGPT + CoT} & N/A & 67.8$_{\pm0.5\hphantom{0}}$ & 63.2$_{\pm2.1\hphantom{0}}$ & 88.5$_{\pm2.5\hphantom{0}}$ & 54.2$_{\pm2.8\hphantom{0}}$ & 17.2 & 61.8\\
\textsc{LLaMA2 7B} & 7B & 37.8$_{\pm1.1\hphantom{0}}$ & 32.0$_{\pm4.4\hphantom{0}}$ & 62.3$_{\pm6.5\hphantom{0}}$ & 21.1$_{\pm3.4\hphantom{0}}$ & 1.5 & 32.4\\
\textsc{LLaMA2 13B} & 13B & 47.7$_{\pm3.0\hphantom{0}}$ & 46.3$_{\pm4.0\hphantom{0}}$ & 80.0$_{\pm2.1\hphantom{0}}$ & 34.4$_{\pm4.7\hphantom{0}}$ & 5.1 & 47.1\\
\textsc{LLaMA2 70B} & 70B & 78.9$_{\pm0.6\hphantom{0}}$ & 64.0$_{\pm4.8\hphantom{0}}$ & 90.6$_{\pm2.5\hphantom{0}}$ & 54.6$_{\pm5.5\hphantom{0}}$ & 21.1 & 63.5\\
\textsc{Mistral 7B} & 7B & 58.2$_{\pm1.6\hphantom{0}}$ & 57.5$_{\pm5.4\hphantom{0}}$ & 88.1$_{\pm3.0\hphantom{0}}$ & 46.7$_{\pm7.3\hphantom{0}}$ & 9.4 & 57.2\\
\multicolumn{8}{c}{\cellcolor{light-gray} \emph{One-Shot on RULE}} \\
%\textsc{UnifiedQA-v2-Base} & 220M & 27.7$_{\pm2.7\hphantom{0}}$ & 36.5$_{\pm2.5\hphantom{0}}$ & 38.5$_{\pm4.0\hphantom{0}}$ & 35.8$_{\pm2.5\hphantom{0}}$ & 1.6 & 36.9\\
%\textsc{UnifiedQA-v2-Large} & 770M & 28.3$_{\pm1.4\hphantom{0}}$ & 27.4$_{\pm1.2\hphantom{0}}$ & 27.4$_{\pm10.2}$ & 27.4$_{\pm3.0\hphantom{0}}$ & 1.0 & 27.7\\
%\textsc{UnifiedQA-v2-3B} & 3B & 35.0$_{\pm1.4\hphantom{0}}$ & 30.1$_{\pm4.8\hphantom{0}}$ & 35.8$_{\pm10.7}$ & 28.2$_{\pm4.0\hphantom{0}}$ & 2.0 & 30.6\\
%\textsc{UnifiedQA-v2-11B} & 11B & 42.6$_{\pm7.1\hphantom{0}}$ & 37.4$_{\pm11.7}$ & 47.5$_{\pm17.7}$ & 33.9$_{\pm9.7\hphantom{0}}$ & 3.1 & 38.0\\
\textsc{Flan-T5-XXL} & 11B & 60.6$_{\pm0.5\hphantom{0}}$ & 64.1$_{\pm3.6\hphantom{0}}$ & 85.8$_{\pm3.1\hphantom{0}}$ & 56.5$_{\pm3.9\hphantom{0}}$ & 14.0 & 63.2\\
\textsc{Flan-UL2} & 20B & 57.6$_{\pm0.4\hphantom{0}}$ & 66.0$_{\pm4.5\hphantom{0}}$ & 87.4$_{\pm3.8\hphantom{0}}$ & 58.5$_{\pm4.7\hphantom{0}}$ & 17.2 & 64.9\\
\textsc{LLaMA 7B} & 7B & 28.2$_{\pm2.4\hphantom{0}}$ & 32.9$_{\pm2.5\hphantom{0}}$ & 48.3$_{\pm8.1\hphantom{0}}$ & 27.4$_{\pm4.1\hphantom{0}}$ & 1.6 & 33.6\\
\textsc{LLaMA 13B} & 13B & 30.0$_{\pm3.2\hphantom{0}}$ & 32.9$_{\pm1.3\hphantom{0}}$ & 50.9$_{\pm4.3\hphantom{0}}$ & 26.6$_{\pm1.8\hphantom{0}}$ & 1.7 & 33.4\\
\textsc{LLaMA 33B} & 33B & 53.3$_{\pm3.2\hphantom{0}}$ & 48.4$_{\pm4.5\hphantom{0}}$ & 79.7$_{\pm3.4\hphantom{0}}$ & 37.3$_{\pm4.7\hphantom{0}}$ & 6.0 & 48.4\\
\textsc{LLaMA 65B} & 65B & 62.8$_{\pm3.4\hphantom{0}}$ & 52.8$_{\pm6.0\hphantom{0}}$ & 84.9$_{\pm4.4\hphantom{0}}$ & 41.5$_{\pm6.5\hphantom{0}}$ & 7.5 & 52.0\\
\textsc{Vicuna 7B} & 7B & 34.7$_{\pm1.8\hphantom{0}}$ & 41.2$_{\pm2.4\hphantom{0}}$ & 65.3$_{\pm6.4\hphantom{0}}$ & 32.6$_{\pm3.3\hphantom{0}}$ & 3.4 & 41.2\\
\textsc{Vicuna 13B} & 13B & 40.7$_{\pm2.3\hphantom{0}}$ & 41.7$_{\pm1.6\hphantom{0}}$ & 67.3$_{\pm4.8\hphantom{0}}$ & 32.7$_{\pm1.8\hphantom{0}}$ & 3.5 & 41.8\\
\textsc{InstructGPT} & N/A & 65.4$_{\pm1.9\hphantom{0}}$ & 66.5$_{\pm1.3\hphantom{0}}$ & 89.0$_{\pm0.8\hphantom{0}}$ & 58.5$_{\pm1.2\hphantom{0}}$ & 19.5 & 65.5\\
\textsc{InstructGPT + CoT} & N/A & 64.3$_{\pm2.5\hphantom{0}}$ & 64.3$_{\pm2.4\hphantom{0}}$ & 88.8$_{\pm1.3\hphantom{0}}$ & 55.7$_{\pm2.5\hphantom{0}}$ & 15.4 & 62.5\\
\textsc{LLaMA2 7B} & 7B & 32.8$_{\pm3.3\hphantom{0}}$ & 33.4$_{\pm1.7\hphantom{0}}$ & 56.1$_{\pm1.8\hphantom{0}}$ & 25.4$_{\pm1.9\hphantom{0}}$ & 1.4 & 34.0\\
\textsc{LLaMA2 13B} & 13B & 45.0$_{\pm5.5\hphantom{0}}$ & 40.9$_{\pm2.9\hphantom{0}}$ & 70.6$_{\pm4.4\hphantom{0}}$ & 30.3$_{\pm2.6\hphantom{0}}$ & 2.8 & 41.1\\
\textsc{LLaMA2 70B} & 70B & 76.0$_{\pm0.2\hphantom{0}}$ & 61.5$_{\pm2.8\hphantom{0}}$ & 90.4$_{\pm3.1\hphantom{0}}$ & 51.4$_{\pm2.7\hphantom{0}}$ & 19.2 & 61.1\\
\textsc{Mistral 7B} & 7B & 50.8$_{\pm1.1\hphantom{0}}$ & 53.8$_{\pm3.3\hphantom{0}}$ & 84.0$_{\pm3.7\hphantom{0}}$ & 43.2$_{\pm3.6\hphantom{0}}$ & 6.5 & 54.0\\
\multicolumn{8}{c}{\cellcolor{light-gray} \emph{Zero-Shot}} \\
%\textsc{UnifiedQA-v2-Base} & 220M & 30.4\hphantom{$_{\pm0.00}$} & 42.2$_{\pm1.0\hphantom{0}}$ & 48.5$_{\pm2.9\hphantom{0}}$ & 39.9$_{\pm1.3\hphantom{0}}$ & 2.7 & 41.7\\
%\textsc{UnifiedQA-v2-Large} & 770M & 41.4\hphantom{$_{\pm0.00}$} & 42.9$_{\pm1.8\hphantom{0}}$ & 55.0$_{\pm4.9\hphantom{0}}$ & 38.5$_{\pm1.3\hphantom{0}}$ & 3.3 & 41.9\\
%\textsc{UnifiedQA-v2-3B} & 3B & 45.5\hphantom{$_{\pm0.00}$} & 47.9$_{\pm2.1\hphantom{0}}$ & 71.6$_{\pm2.9\hphantom{0}}$ & 39.4$_{\pm2.2\hphantom{0}}$ & 5.7 & 47.8\\
%\textsc{UnifiedQA-v2-11B} & 11B & 55.2\hphantom{$_{\pm0.00}$} & 57.3$_{\pm2.7\hphantom{0}}$ & 74.8$_{\pm5.2\hphantom{0}}$ & 51.1$_{\pm2.7\hphantom{0}}$ & 9.7 & 56.5\\
\textsc{Flan-T5-XXL} & 11B & 60.0\hphantom{$_{\pm0.00}$} & 64.3$_{\pm4.0\hphantom{0}}$ & 86.2$_{\pm5.4\hphantom{0}}$ & 56.5$_{\pm3.3\hphantom{0}}$ & 14.7 & 63.4\\
\textsc{Flan-UL2} & 20B & 56.2\hphantom{$_{\pm0.00}$} & 65.7$_{\pm5.2\hphantom{0}}$ & 84.5$_{\pm4.4\hphantom{0}}$ & 59.1$_{\pm5.1\hphantom{0}}$ & 14.7 & 64.2\\
\textsc{LLaMA 7B} & 7B & 27.7\hphantom{$_{\pm0.00}$} & 27.4$_{\pm4.1\hphantom{0}}$ & 38.2$_{\pm4.2\hphantom{0}}$ & 23.6$_{\pm4.6\hphantom{0}}$ & 0.8 & 27.1\\
\textsc{LLaMA 13B} & 13B & 31.7\hphantom{$_{\pm0.00}$} & 36.0$_{\pm3.3\hphantom{0}}$ & 59.3$_{\pm2.1\hphantom{0}}$ & 27.8$_{\pm3.7\hphantom{0}}$ & 1.4 & 36.7\\
\textsc{LLaMA 33B} & 33B & 54.5\hphantom{$_{\pm0.00}$} & 50.9$_{\pm4.4\hphantom{0}}$ & 81.3$_{\pm2.8\hphantom{0}}$ & 40.1$_{\pm4.5\hphantom{0}}$ & 6.8 & 50.9\\
\textsc{LLaMA 65B} & 65B & 52.1\hphantom{$_{\pm0.00}$} & 47.9$_{\pm3.1\hphantom{0}}$ & 78.9$_{\pm1.8\hphantom{0}}$ & 36.9$_{\pm3.5\hphantom{0}}$ & 5.4 & 47.2\\
\textsc{Vicuna 7B} & 7B & 36.7\hphantom{$_{\pm0.00}$} & 40.5$_{\pm2.3\hphantom{0}}$ & 73.1$_{\pm3.2\hphantom{0}}$ & 28.9$_{\pm2.9\hphantom{0}}$ & 2.4 & 40.1\\
\textsc{Vicuna 13B} & 13B & 44.2\hphantom{$_{\pm0.00}$} & 49.5$_{\pm2.7\hphantom{0}}$ & 77.1$_{\pm1.7\hphantom{0}}$ & 39.7$_{\pm2.7\hphantom{0}}$ & 6.2 & 49.4\\
\textsc{InstructGPT} & N/A & 64.1\hphantom{$_{\pm0.00}$} & 62.8$_{\pm2.2\hphantom{0}}$ & 89.9$_{\pm2.0\hphantom{0}}$ & 53.2$_{\pm2.1\hphantom{0}}$ & 15.5 & 61.8\\
\textsc{InstructGPT + CoT} & N/A & 63.8\hphantom{$_{\pm0.00}$} & 62.3$_{\pm1.0\hphantom{0}}$ & 89.6$_{\pm1.5\hphantom{0}}$ & 52.6$_{\pm1.5\hphantom{0}}$ & 14.2 & 61.2\\
\textsc{LLaMA2 7B} & 7B & 32.3\hphantom{$_{\pm0.00}$} & 35.9$_{\pm3.9\hphantom{0}}$ & 66.4$_{\pm4.7\hphantom{0}}$ & 25.1$_{\pm3.4\hphantom{0}}$ & 2.5 & 36.3\\
\textsc{LLaMA2 13B} & 13B & 43.8\hphantom{$_{\pm0.00}$} & 44.4$_{\pm3.0\hphantom{0}}$ & 75.3$_{\pm3.1\hphantom{0}}$ & 33.5$_{\pm2.5\hphantom{0}}$ & 4.7 & 44.5\\
\textsc{LLaMA2 70B} & 70B & 70.8\hphantom{$_{\pm0.00}$} & 58.0$_{\pm3.7\hphantom{0}}$ & 88.1$_{\pm3.4\hphantom{0}}$ & 47.3$_{\pm4.0\hphantom{0}}$ & 14.1 & 57.3\\
\textsc{Mistral 7B} & 7B & 54.0\hphantom{$_{\pm0.00}$} & 55.9$_{\pm3.2\hphantom{0}}$ & 85.9$_{\pm2.0\hphantom{0}}$ & 45.3$_{\pm3.6\hphantom{0}}$ & 8.6 & 55.0\\
\midrule \textsc{Human} & - & \textbf{91.5}\hphantom{$_{\pm0.00}$} & \textbf{82.6}\hphantom{$_{\pm0.00}$} & \textbf{93.0}\hphantom{$_{\pm0.00}$} & \textbf{78.9}\hphantom{$_{\pm0.00}$} & \textbf{52.9} & \textbf{81.5} \\   
\bottomrule
\end{tabular}
